The ETH-MAV Team in the MBZ International Robotics Challenge

This article describes the hardware and software systems of the Micro Aerial Vehicle (MAV) platforms used by the ETH Zurich team in the 2017 Mohamed Bin Zayed International Robotics Challenge (MBZIRC). The aim was to develop robust outdoor platforms with the autonomous capabilities required for the competition, by applying and integrating knowledge from various fields, including computer vision, sensor fusion, optimal control, and probabilistic robotics. This paper presents the major components and structures of the system architectures, and reports on experimental findings for the MAV-based challenges in the competition. Main highlights include securing second place both in the individual search, pick, and place task of Challenge 3 and the Grand Challenge, with autonomous landing executed in less than one minute and a visual servoing success rate of over 90% for object pickups.

==> Makefile <==
# The target that we want to build, TODO: change name if required
targets=main.pdf

# Dependencies, all files which are taken into consideration when make decides
# if rebuilding is necessary
deps=$(wildcard */*.tex) $(wildcard img/*.png) $(wildcard img/*.jpg) \
	$(wildcard img/*.jpeg) $(wildcard img/*.pdf) \
	$(wildcard *.bib)

# NOTE: you should not change anything below
%.pdf: %.tex $(deps) Makefile build
	# Convert eps to pdf.
	# cd build/img && cp ../../img/*.eps ./
	# cd to build and build the report
	cd build && TEXINPUTS=../:../packages:${TEXINPUTS}:. pdflatex $<
	cd build && BIBINPUTS=../:${BIBINPUTS} BSTINPUTS=../:${BSTINPUTS} bibtex $*
	cd build && TEXINPUTS=../:../packages:${TEXINPUTS}:. pdflatex $<
	cd build && TEXINPUTS=../:../packages:${TEXINPUTS}:. pdflatex $<
	# copy the resulting pdf back to the main directory (mv is no good, because
	# make will rebuild even if nothing has changed)
	cp build/$@ .

all: $(targets)

clean: buildclean

build:
	# make sure that build exists
	mkdir -p build
	mkdir -p build/img

buildclean:
	# remove the build folder
	rm -rf build *~ */*~

distclean: clean
	# remove the build folder (clean) and the target pdf
	rm -f $(targets)

installdeb:
	# required packages to use this makefile
	sudo apt-get install texlive texlive-math-extra texlive-publishers

.PHONY: clean buildclean distclean all dist installdeb

